Soft Swing-up: Benchmarking Model-Based Optimal Control for Rigid-Soft Underactuated Systems

Continuum soft robots are inherently underactuated and subject to intrinsic input constraints, making dynamic control particularly challenging, especially in hybrid rigid-soft robots. While most existing methods focus on quasi-static behaviors, dynamic tasks such as swing-up require accurate exploitation of continuum dynamics. This has led to studies on simple low-order template systems that often fail to capture the complexity of real continuum deformations. Model-based optimal control offers a systematic solution; however, its application to rigid-soft robots is often limited by the computational cost and inaccuracy of numerical differentiation for high-dimensional models. Building on recent advances in the Geometric Variable Strain model that enable analytical derivatives, this work investigates three optimal control strategies for underactuated soft systems -- Direct Collocation, Differential Dynamic Programming, and Nonlinear Model Predictive Control -- to perform dynamic swing-up tasks. To address stiff continuum dynamics and constrained actuation, implicit integration schemes and warm-start strategies are employed to improve numerical robustness and computational efficiency. The methods are evaluated in simulation on three Rigid-Soft and high-order soft benchmark systems -- the Soft Cart-Pole, the Soft Pendubot, and the Soft Furuta Pendulum -- highlighting their performance and computational trade-offs.

==> algorithms/box_iddp_algorithm.tex <==
\begin{algorithm}[t]
\caption{\ac{Box-IDDP}}
\label{alg:box_iddp}
\begin{algorithmic}[1]
% Input
\Require Initial state $\bm{x}_0$, initial guess $\bm{U} = \{\bm{u}_0, \dots, \bm{u}_{N-1}\}$
\Ensure Optimal trajectories $\bm{X}^*, \bm{U}^*$
\State Rollout nominal trajectory $\bm{X}, \bm{U}$ by solving $\bm{g}(\bm{x}_{k+1}, \bm{x}_k, \bm{u}_k) = 0$
\Repeat
    \State \Comment{\textit{Backward Pass}}
    \State Initialize $\bm{V}_{\bm{x}} = \bm{l}_{f, \bm{x}}(\bm{x}_N)$ and $\bm{V}_{\bm{x}\bm{x}} = \bm{l}_{f, \bm{x}\bm{x}}(\bm{x}_N)$
    \For{$k = N-1$ \textbf{downto} $0$}
        \State Compute $Q$-derivatives via \eqref{eq:Qx}-\eqref{eq:Qux}.
        \State $[\bm{l}_k, \, \bm{L}_k] \gets \text{Box-QP}\left(\delta \bm{x}_k, \bm{u}_{\text{lb}}, \bm{u}_{\text{ub}}\right)$
        \State $\bm{V}_x \gets \bm{Q}_x - \bm{L}_k^\top \bm{Q}_{uu} \bm{l}_k$
        \State $\bm{V}_{xx} \gets \bm{Q}_{xx} - \bm{L}_k^\top \bm{Q}_{uu} \bm{L}_k$
    \EndFor
    \State \Comment{\textit{Forward Pass \& Line Search}}
    \State \textbf{Define:} $\text{clamp}\left(\bm{u}\right) = \max\left\{\bm{u}_{\text{lb}}, \min\left\{\bm{u}_{\text{ub}}, \bm{u}\right\}\right\}$
    \State $\alpha \gets 1$
    \While{True}
        \State $\hat{\bm{x}}_0 \gets \bm{x}_0$
        \For{$k = 0$ \textbf{to} $N-1$}
            \State $\hat{\bm{u}}_k \gets \text{clamp}\left(\bm{u}_k + \alpha \bm{l}_k + \bm{L}_k(\hat{\bm{x}}_k - \bm{x}_k)\right)$
            \State Solve $\bm{g}(\hat{\bm{x}}_{k+1}, \hat{\bm{x}}_k, \hat{\bm{u}}_k) = 0$ for $\hat{\bm{x}}_{k+1}$.
        \EndFor
        
        \Comment{\textit{Cost improvement}}
        \If{$J(\hat{\bm{X}}, \hat{\bm{U}}) < J(\bm{X}, \bm{U})$} 
            \State $\bm{X} \gets \hat{\bm{X}}$, $\bm{U} \gets \hat{\bm{U}}$
            \State \textbf{break}
        \EndIf
        \State $\alpha \gets 0.5 \alpha$
    \EndWhile
\Until{convergence criteria met}
\State \Return $\bm{X}, \bm{U}$
\end{algorithmic}
\end{algorithm}

==> algorithms/warm_start_algorithm.tex <==
\begin{algorithm}[t]
\caption{Warm-Start Strategy}
\label{alg:warm_start}
\begin{algorithmic}[1]
    \Require Initial state $\bm{x}_0$, target state $\bm{x}_{\text{target}}$, initial guess $\bm{U}_{\text{ig}} = \{\bm{u}_0, \dots, \bm{u}_{N-1}\}$, max truncation order $N_{\max}$
    \Ensure Optimal trajectories $\bm{X}^*, \bm{U}^*$
    
    \State \Comment{\textit{Step 1: Rigid-Body Optimization}}
    \State $\mathcal{M}_{\text{rigid}} \gets$ Equivalent Rigid Model
    \State $\bm{X}, \bm{U}_{\text{init}} \gets \text{TO}(\mathcal{M}_{\text{rigid}}, \bm{U}_{\text{ig}})$
    
    \State \Comment{\textit{Step 2: Progressive Curvature Activation}}
    \For{$n = 0$ \textbf{to} $N_{\max}$}
        \State $\mathcal{M}_{\text{soft}} \gets$ Enable curvature modes at order $n$
        \State $\bm{X}, \bm{U}_{\text{init}} \gets \text{TO}(\mathcal{M}_{\text{soft}}, \bm{U}_{\text{init}})$
    \EndFor
    
    \State \Comment{\textit{Step 3: Full Model with Linear Strain modes}}
    \State $\mathcal{M}_{\text{full}} \gets$ Enable linear strain modes at order $N_{\max}$
    \State $\bm{X}^*, \bm{U}^* \gets \text{TO}(\mathcal{M}_{\text{full}}, \bm{U}_{\text{init}})$
    
    \State \Return $\bm{X}^*, \bm{U}^*$
\end{algorithmic}
\end{algorithm}

==> sections/rebuttal.tex <==
\noindent We thank the Area Chair~(5rJP) and the Reviewers~(Wq3G, JA1E, WtYu, RekB) for their careful reading and constructive feedback. We clarify several key points below.

\vspace{0.5em}

\noindent \textbf{1. Clarification of Contribution and Novelty}:
The primary contribution of this work lies in enabling model-based optimal control for underactuated rigid-soft systems. Specifically, we achieve this for 3D, dynamic, and high-order continuum models performing tasks at unstable equilibria (such as the swing-up task). To the best of the authors' knowledge, this is the first demonstration of such capabilities in the soft robotics literature without relying on quasi-static or pseudo-rigid approximations.

To successfully control these complex continuum dynamics, we found that existing model-based optimal controllers (\acs{DC}, \acs{DDP}, and \acs{NMPC}) require specific adaptations to handle stiff differential equations and intrinsic actuation limits. Therefore, the \acs{Box-IDDP} algorithm and the resolution-based warm-start strategy are proposed precisely to overcome these bottlenecks. 

\textcolor{red}{We improved Sec. II-D of the manuscript to clarify the contributions of this work.}

\noindent \textbf{2. Clarification on \acs{DC} as baseline method~(Wq3G)}:
\acs{DC} serves as a baseline for evaluating \acs{Box-IDDP} using the same \acs{GVS} model, but the application of \acs{DC} itself is also a contribution. Solving optimal control problems for high-order rigid-soft systems is challenging; we formulate \acs{DC} as a large-scale \acs{NLP} using exact analytical GVS derivatives to enable complex motions such as the swing-up task. While \acs{Box-IDDP} is more efficient and robust in closed-loop settings, \acs{DC} excels in offline trajectory planning with complex, non-convex constraints (e.g., collision avoidance). 

\textcolor{red}{We revised Section IV-B and Section V-D to explicitly reflect these points.}

\noindent \textbf{3. Clarification on ``desired fidelity"~(WtYu)}:
We clarified this concept (referred to as ``desired fidelity" in the original submission) to mean the specific ``desired truncation" of the infinite-dimensional strain field required in \acs{GVS} to accurately capture continuum dynamics. This truncation is systematically adjusted by increasing the order of the Legendre polynomial basis. In our models, the ``desired truncation" corresponds to a \textit{second-order Legendre polynomial} expansion for curvature and linear strain modes (3 \acs{DoFs} per mode).
We highlight this level because it enables a degree of shape complexity that was not achieved before by constant (Webster et al. 2010) or affine curvature (Della Santina, 2020) models.

\textcolor{red}{We added the algorithm box of the warm-start strategy and clarified this point in Sec. IV-E.}

\noindent \textbf{4. Mathematical Formalization of Warm-Start~(WtYu)}:
We must clarify that, due to the highly non-convex nature of the trajectory optimization problem for high-DoF continuum models, providing a formal analytical proof of global convergence or guaranteeing the absence of local minima is theoretically intractable. To the best of our knowledge, such guarantees do not currently exist in the literature for \acs{DDP} or \acs{NMPC} applied to highly nonlinear soft robotic systems.

However, our warm-start strategy exploits the GVS mathematical structure: strain fields are parameterized via truncated Legendre polynomial expansions. As the polynomial order increases, higher-order terms have diminishing influence on the overall dynamics. Thus, a reduced-order optimal trajectory provides an effective initial guess for higher-order models. While not an analytical guarantee, this approach systematically positions the solver closer to the optimum, empirically accelerating convergence (Fig. 6a). 

\textcolor{red}{We included this consideration in Sec. IV-E.}

\noindent \textbf{5. Comparison with alternative Dynamic Models~(Wq3G)}:
While a direct numerical benchmark is beyond the scope of this work, we added a discussion comparing \acs{GVS} with alternative dynamic models, highlighting its advantages for \acs{TO}.
%
\acs{PCC}~(Webster et al., 2010) is computationally efficient but cannot capture continuous strain (bending, shear, twisting); we use it only to generate warm-start initial guesses. Cosserat rod models~(Till et al., 2019) achieve real-time forward dynamics via shooting methods, but embedding them in optimal control makes analytical gradient computation extremely challenging. \acs{GVS} overcomes this by parameterizing the strain field, reducing \acsp{PDE} to \acsp{ODE}.
%
Spatial discretization frameworks like \acs{DER}~(Gazzola et al., 2018) and DEFORM~(Chen et al., 2024) provide real-time performance but rely on position-based formulations that increase \acs{OCP} dimensionality, with DEFORM additionally assuming inextensibility.
%
Crucially, \acs{GVS} extends the geometric theory of rigid robots to hybrid systems featuring both rigid joints and Cosserat rods, allowing us to naturally handle rigid-soft interactions and directly leverage well-established rigid-body algorithms for trajectory optimization. 

\textcolor{red}{We provided this discussion in Sec. II.}

\noindent \textbf{6. Clarification on Warm-start Computational Time~(JA1E)}:
Figure 6c reports the average computational time per iteration of \acs{DC} and \acs{Box-IDDP} using a pseudo-random initial guess for both methods.
While including the warm-start cost makes the proposed approach slower, random initializations frequently cause solver failures or poor local minima—leaving the robot stationary or far from the target, especially in complex underactuated systems.

Thus, the warm-start approach is well-suited for offline \acs{TO}. For \acs{NMPC}, it can be used to initialize the first solution to improve target convergence without compromising subsequent real-time performance.

\textcolor{red}{We clarified this point in Sec. IV-E.}

\noindent \textbf{7. Minor Revisions~(5rJP, Wq3G, JA1E, WtYu, RekB)}:
As suggested, we: (i) added an algorithm box for \acs{Box-IDDP} and the warm-start strategy in the Supplementary Material, (ii) increased the font size of the figures, (iii) included the final error as a metric, (iv) improved the abstract as suggested, and (v) reduced the use of acronyms. Finally, we emphasized the limitations of FEM and Koopman-based approaches in the related works section.

\vspace{0.5em}

\noindent We hope these clarifications address the concerns and improve the clarity of the paper.

==> tables/soft_link.tex <==
\begin{table}
\centering
\caption{Geometrical and physical parameters of a Soft Link}
\label{tab:soft_link_params}
    \begin{tabular}{lll}
    \toprule
    Name                    &   Symbol          &   Value                                                               \\
    \midrule
    Length                  &   $L$               &   \SI{1.0}{\meter}                                                            \\
    Cross-Section Radius               &   $R_{\textnormal{cs}}$               &   \SI{0.03}{\meter}                                                            \\
    Density                 &   $\bar{\rho}$    &   \SI{1000.0}{\kilogram/\meter^3}                                     \\     
    Young's Modulus         &   $E$             &   \SI{1.0}{M\pascal}                                             \\
    Poisson Ratio           &   $\nu$           &   0.5                                                                     \\
    Damping Coefficient                &   $\beta$         &   \SI{0.01}{M\pascal \cdot \second}         \\
    Stress-Free Strain      & $\bm{\xi}^{*}$    &   $[0, \, 0, \, 0, \, 1, \, 0, \, 0]^{\top}$    \\
    Joint Damping & $\beta_r$ & $\SI[inter-unit-product =$\cdot$]{0.05}{\newton\meter\second/\radian}$ \\ 
    \bottomrule
    \end{tabular}
\end{table}
